Categorization in the Wild: Generalizing Cognitive Models to Naturalistic Data across Languages

Categories such as animal or furniture are acquired at an early age and play an important role in processing, organizing, and communicating world knowledge. Categories exist across cultures: they allow to efficiently represent the complexity of the world, and members of a community strongly agree on their nature, revealing a shared mental representation. Models of category learning and representation, however, are typically tested on data from small-scale experiments involving small sets of concepts with artificially restricted features; and experiments predominantly involve participants of selected cultural and socio-economical groups (very often involving western native speakers of English such as U.S. college students) . This work investigates whether models of categorization generalize (a) to rich and noisy data approximating the environment humans live in; and (b) across languages and cultures. We present a Bayesian cognitive model designed to jointly learn categories and their structured representation from natural language text which allows us to (a) evaluate performance on a large scale, and (b) apply our model to a diverse set of languages. We show that meaningful categories comprising hundreds of concepts and richly structured featural representations emerge across languages. Our work illustrates the potential of recent advances in computational modeling and large scale naturalistic datasets for cognitive science research.

==> figures/bcf-vs-strudel-types.tex <==
\noindent\fbox{%
\begin{varwidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}
 \resizebox{\columnwidth}{!}{
  \begin{tikzpicture}
 
 \tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=0pt and 0pt of #1.south east] %

\tikzstyle{every node}=[ellipse, maximum width=10pt,
    align=center]
 
  % Nodes
  \node[draw, ellipse, align=center]         (B0)     {\bf$\ \ $ BCF $\ \ $} ; %
  \node[draw, ellipse, align=center, right=0.5cm of B0]       (B1)     {hand foot leg\\ finger  arm} ; %
  \node[draw, ellipse, align=center, right=0.5cm of B1]       (B2)     {kill door hand\\ break cut} ; %
  \node[draw, ellipse, align=center, right=0.5cm of B2]       (B3)     {woman dress shirt\\ clothing  shoe} ; %
  \node[draw, ellipse, align=center, right=0.5cm of B3]       (B4)     {ball goal score \\field touchdown} ; %
  \node[draw, ellipse, align=center, right=0.5cm of B4]       (B5)     {tail bird leg\\ wing foot} ; %
  
  \node[draw, ellipse, align=center, below=1cm of B0] (S0)     {\bf Strudel} ; %
  \node[draw, ellipse, align=center, right=0.5cm of S0]       (S1)     {feed leg tight\\ transform left}; %
  \node[draw, ellipse, align=center, right=0.5cm of S1]       (S2)     {record grow rate\\conduct service } ; %
  \node[draw, ellipse, align=center, right=0.5cm of S2]       (S3)     {fiber magic label\\ brand equipment} ; %
  \node[draw, ellipse, align=center, right=0.5cm of S3]       (S4)     {pain bed gun\\stay knee} ; %
  \node[draw, ellipse, align=center, right=0.5cm of S4]       (S5)     {pattern air cup\\ victory marker } ; %
  
  \node[draw, ellipse, align=center, below=1cm of S0]         (C0)     {\bf Co-occ } ; %
  \node[draw, ellipse, align=center, right=0.5cm of C0]       (C1)     {pop discipline\\ shock lick race} ; %
  \node[draw, ellipse, align=center, right=0.5cm of C1]       (C2)     {base animal defined\\ embroider painting} ; %
  \node[draw, ellipse, align=center, right=0.5cm of C2]       (C3)     {patient collapse\\ amputate leg joint} ; %
  \node[draw, ellipse, align=center, right=0.5cm of C3]       (C4)     {rail trail memory\\ forward meter} ; %
  \node[draw, ellipse, align=center, right=0.5cm of C4]       (C5)     {abdomen fight bend\\powerful slice} ; %
  \end{tikzpicture}
 }
 \end{varwidth}
 }
